L-Recursion and a new Logic for Logarithmic Space

We extend first-order logic with counting by a new operator that allows it to formalise a limited form of recursion which can be evaluated in logarithmic space. The resulting logic LREC has a data complexity in LOGSPACE, and it defines LOGSPACE-complete problems like deterministic reachability and Boolean formula evaluation. We prove that LREC is strictly more expressive than deterministic transitive closure logic with counting and incomparable in expressive power with symmetric transitive closure logic STC and transitive closure logic (with or without counting). LREC is strictly contained in fixed-point logic with counting FPC. We also study an extension LREC= of LREC that has nicer closure properties and is more expressive than both LREC and STC, but is still contained in FPC and has a data complexity in LOGSPACE. Our main results are that LREC captures LOGSPACE on the class of directed trees and that LREC= captures LOGSPACE on the class of interval graphs.

==> pic_mod_decomp.tex <==



\begin{figure}%[h]
%\vspace{.5cm}
\centering
\begin{tikzpicture}[intvl/.style={|-|,shorten >=-.7pt,shorten <=-.7pt},
                    v/.style={circle,inner sep=0pt,minimum size=4pt},
        			e/.style={->, shorten >=1pt}]

\begin{scope}[xshift=-4.5cm,scale=.9]

  \foreach \x in {1,...,11}
 {
  \fill[xshift=\x cm-1cm,rounded corners=1pt,fill=gray!20!white] (-3pt,-.3cm) rectangle (3pt,2.3cm);
  \draw[xshift=\x cm-1cm] (0,-.3cm) node[anchor=north] {\small $M_{\x}$};
 }

\filldraw (0,0) node[anchor=east] {\small $a$} circle (1.5pt)
    (10,0) node[anchor=west] {\small $e$} circle (1.5pt)
    (1,0) node[anchor=west] {\small $f$} circle (1.5pt)
    (2,0) node[anchor=west] {\small $g$} circle (1.5pt)
    (3,0) node[anchor=west] {\small $j$} circle (1.5pt)
    (4,0) node[anchor=east] {\small $m$} circle (1.5pt)
    (5,0) node[anchor=west] {\small $n$} circle (1.5pt)
    (6,0) node[anchor=west] {\small $s$} circle (1.5pt)
    (7,0) node[anchor=west] {\small $t$} circle (1.5pt)
    (8,0) node[anchor=west] {\small $u$} circle (1.5pt)
    (9,0) node[anchor=west] {\small $r$} circle (1.5pt);

\draw[intvl] (0,1.5) -- (3,1.5) node[midway,above,inner sep=1pt] {\small $b$};
\draw[intvl] (1,2) -- (9,2) node[near start,above,inner sep=1pt] {\small $c$};
\draw[intvl] (6,1.5) -- (10,1.5) node[very near start,above,inner sep=1pt] {\small $d$};
\draw[intvl] (2,.4) -- (3,.4) node[midway,above,inner sep=1pt] {\small $h$};
\draw[intvl] (4,.4) -- (5,.4) node[midway,below,inner sep=1pt] {\small $l$};
\draw[intvl] (4,.7) -- (5,.7) node[midway,above,inner sep=1pt] {\small $k$};
\draw[intvl] (6,.5) -- (8,.5) node[near start,above,inner sep=1pt] {\small $o$};
\draw[intvl] (7,.7) -- (9,.7) node[near end,below,inner sep=1pt] {\small $q$};
\draw[intvl] (7,1) -- (9,1) node[near end,above,inner sep=1pt] {\small $p$};

\end{scope}


\begin{scope}[yshift=-3cm]

\node (root) at (0,1.5) {\small $s_V$};
\node (vVentry) at (0,1) {};
\node (vV) at (0,-.8) {};%{\small $v_V$};
\node (vVlabel) at (-1.7,.7) {\small $v_V$};
\draw[draw=gray,rounded corners = 3pt] (-2,-.8) rectangle (2,1);
\node (lM16) at (-4.5,-1.6) {\small $a_{{\{\prec_{M_i}\},V}}\ {\footnotesize (i\leq 4)}$};
\node (lM56) at (0,-1.6) {\small $a_{{\{\prec_{M_i}\},V}}\ (i=5,6)$};
\node (lM66) at (4.5,-1.6) {\small $a_{{\{\prec_{M_i}\},V}}\ (i\geq 7)$};

\draw[->,shorten >=-2pt] (root) -- (vVentry);
\draw[e] (vV) -- (lM16);
\draw[e] (vV) -- (lM56);
\draw[e] (vV) -- (lM66);


\node (sfghi) at (-4.5,-2.4) {\small $s_{\{f,g,h,j\},V}$};
%\node (shij16) at  (-4,-2.6) {\small $s_{\{hij\},L_{M_1,6}}$};
\node (vf) at (-5.5,-3) {}; % {\small $v_{\{f\}}$};
\node (vghi) at (-3.5,-3) {}; % {\small $v_{\{g,h,i\}}$};
\node (vfLabel) at (-5.5,-3.3) {\small $v_{\{f\}}$};
\node (vghiLabel) at (-3.5,-3.3) {\small $v_{\{g,h,j\}}$};
\draw[rounded corners=3pt,draw=gray] (-5.9,-4.6) rectangle (-5.1,-3);
\draw[rounded corners=3pt,draw=gray] (-4.1,-4.6) rectangle (-2.9,-3);

\draw[e] (lM16) -- (sfghi);
\draw[e] (sfghi) -- (vf);
\draw[e] (sfghi) -- (vghi);

\node (vghiOut) at (-3.5,-4.6) {};
\node (aghi) at (-4.1,-5.5) {\small $a_{\{\prec_{M_i  }\},\{g,h,j \} }\ (i=3,4)$};
\node (sgi) at (-4.1,-6.3) {\small $s_{\{g,j\},\{g,h,j \}}$};
\node (vg) at (-4.7,-7.1) {};
\node (vi) at (-3.5,-7.1) {};
\draw[rounded corners=3pt,draw=gray] (-5.1,-8) rectangle (-4.3,-7);
\draw[rounded corners=3pt,draw=gray] (-3.9,-8) rectangle (-3.1,-7);
\draw[e] (vghiOut) -- (aghi);
\draw[e] (aghi) -- (sgi);
\draw[e] (sgi) -- (vg);
\draw[e] (sgi) -- (vi);


\node (sjkl) at (0,-2.4) {\small $s_{\{k,l,m,n\},V}$};
\node (vjkl) at (0,-3) {}; %{\small $v_{\{j,k,l\}}$};
\node (vjklLabel) at (0,-3.3) {\small $v_{\{k,l,m,n\}}$};
\draw[rounded corners=3pt,draw=gray] (-.7,-4.6) rectangle (.7,-3);
\draw[e] (lM56) -- (sjkl);
\draw[->,shorten >=-2pt] (sjkl) -- (vjkl);


\node (vjklOut) at (0,-4.6) {};
\node (ajklm) at (0,-5.5) {\small $a_{\{\prec_{M_i}\}, \{k,l,m,n \}  }\ (i=5,6)$};
\node (sjm) at (0,-6.3) {\small $s_{\{m,n\},\{k,l,m,n\}}$};
\node (vj) at (-.6,-7.1) {};
\node (vm) at (.6,-7.1) {};
\draw[rounded corners=3pt,draw=gray] (-1,-8) rectangle (-.2,-7);
\draw[rounded corners=3pt,draw=gray] (.2,-8) rectangle (1,-7);
\draw[e] (vjklOut) -- (ajklm);
\draw[e] (ajklm) -- (sjm);
\draw[e] (sjm) -- (vj);
\draw[e] (sjm) -- (vm);



\node (smnopqrs) at (4.5,-2.4) {\small $s_{\{o,p,q,r,s,t,u\},V}$};
\node (vmnopqrs) at (4.5,-3) {};% {\small $v_{\{m,n,o,p,q,r,s\}}$};
\node (vmnopqrsExit) at (4.5,-4.8) {};
\node at (4.4,-3.3) {\small $v_{\{o,p,q,r,s,t,u\}}$};
\draw[rounded corners=3pt,draw=gray] (3.25,-4.8) rectangle (5.75,-3);
\node (amnopqrs) at (4.5,-5.5) {\small $a_{\{\prec_{M_i}\},\{o,p,q,r,s,t,u\}}\ (7\leq i\leq 10)$};
\node (srs) at (4.5,-6.3) {\small $s_{\{t,u\},\{o,p,q,r,s,t,u\}}$};
\node (vr) at (3.9,-7.1) {}; % {\small $v_{\{r\}}$};
\node (vs) at (5.1,-7.1) {}; % {\small $v_{\{s\}}$};
\node (vrLabel) at (3.9,-7.3) {\small $v_{\{t\}}$};
\node (vsLabel) at (5.1,-7.3) {\small $v_{\{u\}}$};
\draw[rounded corners=3pt,draw=gray] (3.5,-8) rectangle (4.3,-7);
\draw[rounded corners=3pt,draw=gray] (4.7,-8) rectangle (5.5,-7);

\draw[e] (lM66) -- (smnopqrs);
\draw[->,shorten >=-2pt] (smnopqrs) -- (vmnopqrs);
\draw[e] (vmnopqrsExit) -- (amnopqrs);
\draw[e] (amnopqrs) -- (srs);
\draw[->] (srs) -- (vr);
\draw[->] (srs) -- (vs);



%% colors of module vertices
\node[fill=gray!20!white,rounded corners=3pt] (sfghiColor) at (-5.9,-2.2) {\scriptsize $\{2,4\}$};
\draw[gray,shorten >=-2pt,shorten <=-2pt] (sfghi) -- (sfghiColor);
\node[fill=gray!20!white,rounded corners=3pt] (sjklColor) at (-1.4,-2.2) {\scriptsize $\{3,3\}$};
\draw[gray,shorten >=-2pt,shorten <=-2pt] (sjkl) -- (sjklColor);
\node[fill=gray!20!white,rounded corners=3pt] (smnopqrsColor) at (2.8,-2.2) {\scriptsize $\{2,4\}$};
\draw[gray,shorten >=-2pt,shorten <=-2pt] (smnopqrs) -- (smnopqrsColor);
\node[fill=gray!20!white,rounded corners=3pt] (srsColor) at (2.7,-6.1) {\scriptsize $\{2\}$};
\draw[gray,shorten >=-2pt,shorten <=-2pt] (srs) -- (srsColor);

\node[fill=gray!20!white,rounded corners=3pt] (sgiColor) at (-5.4,-6.1) {\scriptsize $\{1\}$};
\draw[gray,shorten >=-2pt,shorten <=-2pt] (sgi) -- (sgiColor);
\node[fill=gray!20!white,rounded corners=3pt] (sjmColor) at (-1.5,-6.1) {\scriptsize $\{1\}$};
\draw[gray,shorten >=-2pt,shorten <=-2pt] (sjm) -- (sjmColor);



\begin{scope}[xshift=3.8cm,yshift=-4.4cm,scale=.75]

%% label for (vmnopqrs)

\foreach \x in {1,...,3}
 {
  \fill[xshift=\x cm-1cm,rounded corners=1pt,fill=gray!20!white] (-3pt,-.3cm) rectangle (3pt,1.2cm);
 }

\filldraw (0,0) node[anchor=east] {} circle (1.5pt)
            (1,0) node[anchor=east] {} circle (1.5pt)
            (2,0) node[anchor=east] {} circle (1.5pt);


\draw[intvl] (0,.3) -- (1,.3) node[midway,above,inner sep=1pt] {};
\draw[intvl] (1,.6) -- (2,.6) node[midway,above,inner sep=1pt] {};
\draw[intvl] (1,.9) -- (2,.9) node[midway,above,inner sep=1pt] {};

\end{scope}



\begin{scope}[xshift=0cm,yshift=-4.2cm,scale=.75]

%% label for (vjkl)

\foreach \x in {1,...,1}
 {
  \fill[xshift=\x cm-1cm,rounded corners=1pt,fill=gray!20!white] (-3pt,-.3cm) rectangle (3pt,.8cm);
 }

\filldraw (0,0) node[anchor=east] {} circle (1.5pt)
            (0,.25) node[anchor=east] {} circle (1.5pt)
		(0,.5) node[anchor=east] {} circle (1.5pt);

\end{scope}


\begin{scope}[xshift=-3.5cm,yshift=-4.2cm,scale=.75]

%% label for (vghi)

\foreach \x in {1,...,1}
 {
  \fill[xshift=\x cm-1cm,rounded corners=1pt,fill=gray!20!white] (-3pt,-.3cm) rectangle (3pt,.8cm);
 }

\filldraw (0,0) node[anchor=east] {} circle (1.5pt)
            (0,.4) node[anchor=east] {} circle (1.5pt);

\end{scope}


\begin{scope}[xshift=-5.5cm,yshift=-4.2cm,scale=.75]

%% label for (vf)

\foreach \x in {1,...,1}
 {
  \fill[xshift=\x cm-1cm,rounded corners=1pt,fill=gray!20!white] (-3pt,-.3cm) rectangle (3pt,.4cm);
 }
\filldraw (0,0) node[anchor=east] {} circle (1.5pt);

\end{scope}


\begin{scope}[xshift=3.9cm,yshift=-7.7cm,scale=.75]

%% label for (vr)

\foreach \x in {1,...,1}
 {
  \fill[xshift=\x cm-1cm,rounded corners=1pt,fill=gray!20!white] (-3pt,-.3cm) rectangle (3pt,.3cm);
 }
\filldraw (0,0) node[anchor=east] {} circle (1.5pt);

\end{scope}

\begin{scope}[xshift=5.1cm,yshift=-7.7cm,scale=.75]

%% label for (vs)

\foreach \x in {1,...,1}
 {
  \fill[xshift=\x cm-1cm,rounded corners=1pt,fill=gray!20!white] (-3pt,-.3cm) rectangle (3pt,.3cm);
 }
\filldraw (0,0) node[anchor=east] {} circle (1.5pt);

\end{scope}

\begin{scope}[xshift=-4.7cm,yshift=-7.7cm,scale=.75]

%% label for (vg)

\node at (0,.6) {\small $v_{\{g\}}$};

\foreach \x in {1,...,1}
 {
  \fill[xshift=\x cm-1cm,rounded corners=1pt,fill=gray!20!white] (-3pt,-.3cm) rectangle (3pt,.3cm);
 }
\filldraw (0,0) node[anchor=east] {} circle (1.5pt);

\end{scope}

\begin{scope}[xshift=-3.5cm,yshift=-7.7cm,scale=.75]

%% label for (vi)

\node at (0,.6) {\small $v_{\{j\}}$};

\foreach \x in {1,...,1}
 {
  \fill[xshift=\x cm-1cm,rounded corners=1pt,fill=gray!20!white] (-3pt,-.3cm) rectangle (3pt,.3cm);
 }
\filldraw (0,0) node[anchor=east] {} circle (1.5pt);

\end{scope}


\begin{scope}[xshift=-.6cm,yshift=-7.7cm,scale=.75]

%% label for (vg)

\node at (0,.6) {\small $v_{\{m\}}$};

\foreach \x in {1,...,1}
 {
  \fill[xshift=\x cm-1cm,rounded corners=1pt,fill=gray!20!white] (-3pt,-.3cm) rectangle (3pt,.3cm);
 }
\filldraw (0,0) node[anchor=east] {} circle (1.5pt);

\end{scope}

\begin{scope}[xshift=.6cm,yshift=-7.7cm,scale=.75]

%% label for (vi)

\node at (0,.6) {\small $v_{\{n\}}$};

\foreach \x in {1,...,1}
 {
  \fill[xshift=\x cm-1cm,rounded corners=1pt,fill=gray!20!white] (-3pt,-.3cm) rectangle (3pt,.3cm);
 }
\filldraw (0,0) node[anchor=east] {} circle (1.5pt);

\end{scope}


\begin{scope}[xshift=-1.4cm,yshift=-.25cm,scale=.75]

%% label for V

\foreach \x in {1,...,5}
 {
  \fill[xshift=\x cm-1cm,rounded corners=1pt,fill=gray!20!white] (-3pt,-.3cm) rectangle (3pt,1.2cm);
 }

\filldraw (0,0) node[anchor=east] {} circle (1.5pt)
            (1,0) node[anchor=east] {} circle (1.5pt)
            (2,0) node[anchor=east] {} circle (1.5pt)
            (3,0) node[anchor=east] {} circle (1.5pt)
            (4,0) node[anchor=east] {} circle (1.5pt);


\draw[intvl] (0,.5) -- (1,.5) node[midway,above,inner sep=1pt] {};
\draw[intvl] (1,1) -- (3,1) node[midway,above,inner sep=1pt] {};
\draw[intvl] (3,.5) -- (4,.5) node[midway,above,inner sep=1pt] {};

\end{scope}

\end{scope}

\end{tikzpicture}
\caption{An interval graph and its coloured modular decomposition tree. Component vertices $v_U$ are represented together with the interval graph $L_U$ labeling them. The colours of module vertices are indicated in the gray fields next to them.}\label{fig:modularTree}
%\vspace{1cm}
\end{figure}
